Generating the Traces You Need: A Conditional Generative Model for Process Mining Data

In recent years, trace generation has emerged as a significant challenge within the Process Mining community. Deep Learning (DL) models have demonstrated accuracy in reproducing the features of the selected processes. However, current DL generative models are limited in their ability to adapt the learned distributions to generate data samples based on specific conditions or attributes. This limitation is particularly significant because the ability to control the type of generated data can be beneficial in various contexts, enabling a focus on specific behaviours, exploration of infrequent patterns, or simulation of alternative 'what-if' scenarios. In this work, we address this challenge by introducing a conditional model for process data generation based on a conditional variational autoencoder (CVAE). Conditional models offer control over the generation process by tuning input conditional variables, enabling more targeted and controlled data generation. Unlike other domains, CVAE for process mining faces specific challenges due to the multiperspective nature of the data and the need to adhere to control-flow rules while ensuring data variability. Specifically, we focus on generating process executions conditioned on control flow and temporal features of the trace, allowing us to produce traces for specific, identified sub-processes. The generated traces are then evaluated using common metrics for generative model assessment, along with additional metrics to evaluate the quality of the conditional generation

==> x2_Background_OLD.tex <==



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% PREVIOUS VERSION - START
{\color{brown}

\subsection*{B. Conditional Variational Autoencoders (CVAEs)}
Autoencoders are neural network architectures used for unsupervised learning tasks~\cite{doi:10.1126/science.1127647}. They consist of an encoder, \(E\), and a decoder, \(D\). The encoder compresses the input data \(x\) into a latent representation \(z\), while the decoder output \(\hat{x}\) should reconstructs the original input from the latent representation. Mathematically, an autoencoder aims to minimize the reconstruction error between the input and the output:
\begin{equation}
\mathcal{L}_{\text{AE}}(x, \hat{x}) = \lVert x - \hat{x} \rVert^2.
\label{eq:ae_loss}
\end{equation}

Variational autoencoders (VAEs) extend the basic autoencoder architecture by learning a latent space that follows a specific probability distribution, typically a Gaussian distribution~\cite{kingma2022autoencoding}. VAEs are trained to maximize the evidence lower bound (ELBO), which consists of the reconstruction loss \eqref{eq:ae_loss} plus a regularization term based on the Kullback-Leibler (KL) divergence between the learned latent distribution and a prior distribution:
\begin{equation}
\mathcal{L}_{\text{VAE}}(x, \hat{x}, \mu, \sigma) = \lVert x - \hat{x} \rVert^2 + \beta \cdot \text{KL}(q(z|x) \Vert p(z))
\label{eq:vae_loss}
\end{equation}
where \(\mu\) and \(\sigma\) are the mean and standard deviation of the learned latent distribution \(q(z|x)\), and \(\beta\) controls the strength of the regularization.

Conditional variational autoencoders (CVAEs) incorporate conditional information into both the encoder and decoder. In CVAEs, both the encoder and decoder take the input data \(x\) and conditioning variables \(c\) as inputs~\cite{NIPS2015_8d55a249}. The encoder generates a latent representation \(z\) that is conditioned on the input data and conditioning variables, while the decoder reconstructs the input data conditioned on both the latent representation and the conditioning variables:
\begin{equation}
\mathcal{L}_{\text{CVAE}}(x, \hat{x}, c, \mu, \sigma) = \lVert x - \hat{x} \rVert^2 + \beta \cdot \text{KL}(q(z|x,c) \Vert p(z|c))
\label{eq:cvae_loss}
\end{equation}
Here, \(q(z|x)\) and \(q(z|x,c)\) represent the learned distributions of latent variables given input data \(x\) with and without conditioning variables \(c\), respectively. \(p(z)\) and \(p(z|c)\) denote the prior distributions of latent variables with and without conditioning, respectively. 

} 
% CLOSING TEXT COLORING
% PREVIOUS VERSION - END
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> x3_Related_work_OLD.tex <==
\alert{Inserisco qualche idea da sistemare.}
In this section we briefly discuss the related works that study generative and resampling methods in PM and in related fields. 
\alert{Non so neanche io quanto valga la pena addentrarsi nell'ambito simulazione, dipende un po' se e con quali metodi ci confrontiamo nella valutazione.}
In recent years significant efforts have been dedicated to the development and evaluation of generative models for event logs, particularly within the simulation domain \cite{}.
In particular three types of models have been identified: data-driven simulation models, deep learning models, and hybrid models that integrate both methods \cite{dsim,rims}.
However, while a comprehensive evaluation framework has been designed to assess the generative quality of the proposed methods, their potential application as resampling techniques in imbalanced prediction tasks has not been considered yet. \alert{(questa frase \`e rischiosa perch\'e implica che potremmo farlo noi. Metterla gi\`u come segue potrebbe essere pi\`u sicuro)}.
However these methods are  primarily designed and assessed based on their ability to faithfully reproduce the processes from which they are derived. In the context of re-sampling application the primary objective shift towards the improvement of the prediction task rather than exact process replication. Consequently some additional variability beyond the training data is actually desirable.

\andrei{I would add some points on the SMOTE variants and why we don't use them here, I remember @Massi you had some motivation for that, too simple, not able to handle categorical.}\alert{yes good point, I put it here temporary}
A collection of over-sampling techniques widely used in imbalanced learning includes SMOTE (Synthetic Minority Over-sampling Technique) \cite{SMOTE} and  its variants (SMOTEN, SMOTENC, ADASYN, etc.).
These tecniques generate new instances in the minority class by ``mixing together'' components of close existing minority samples.
In detail, after defining a metric in the feature space, the new instance is obtained by selecting an existing sample and its $k$-nearest neighbours within the minority class. The continuous and nominal features of the new instance are obtained, respectively, by interpolation with a random sample chosen among the selected $k$ neighbours and by consensum with the selected $k$ neighbours. 

Conditional Variational Autoencoders (CVAEs) have ben previously used in the literature to solve the class imbalance problem~\cite{FAJARDO2021114463} and improve the performance of classifiers, showing improvements over state-of-the-art resampling techniques.

However these techniques are not directly applicable to process event data for two main reasons: (1) existing techniques use metrics that consider exclusively either continuous or nominal features in the definition of the distance between samples; (2) even when they explicitly use nominal features in the definition of the metric in the feature space (SMOTEN), all nominal feature are threated as independent variables.
Therefore, these approaches are ill-suited for process event data, whose main component---the control flow---is described by nominal features (activity labels). These features are equally, if not more, important than the continuous data payload and possess strong interdepency and causal relations. Hence, some effort to adapt them to this context would be necessary.
\alert{Ovviamente cos\`i \`e un po' lunghetta}


Resampling techniques have been extensively studied in the domain of time series \cite{Jurman,...}, where various techniques such as VAE, GANS, etc., have been applied.
Both process event data and times series involve temporal data, thus indicating a special emphasis on the causal relationships within the data. However time series typically focus on the evolution of continuos variables, whereas process data deals with sequences of nominal features, namely activity labels. Consequently, methods developed for time series cannot be directly applied to event data, but need some adaptation.

To our knowledge only one study \cite{Kappel} has addressed data augmentation for PPM tasks.
In this study the authors employed \emph{simple noise-based transformations} to augment datasets, aiming to enhance the performances of deep learning based PPM tasks, specifically next activity prediction, where the original training dataset is small with respect to the number of parameter of the predictive model.
In contrast to this approach, we propose a novel method for data augmentation to tackle imbalanced prediction problems, leveraging a conditional variational autoencoder architecture.





==> x6_Results_OLD.tex <==
In this section, we present the results obtained.\footnote{\alert{Codice e risultati extra sono nel repo! link}}
We start by showcasing an example of conditional generation with \cvae, in Table~\ref{tab:generation} we list the control-flow of two pairs of traces generated for the experiment \fines. Every pair of traces are generated by the same value of the latent variable $z$ but with different values of the conditional variable $c$.
These two examples are very interesting can be interpretable as ``what-if'' scenarios. When $c=\text{F}$, in both cases the fine is paid by the offender within a short time. When $c=\text{F}$, the offender appeals to the Judge and to the Prefecture respectively. This causes delays, and as a consequence, a penalty is added after six months from the issuance of the fine, and this is known to be a process constraint \cite{traffic_fines_report} \massi{(we will show answering \ref{RQ3} that  the robustness under process constraint is not an accident of this example, but is a general feature of our model)}.
The first example ends with the \emph{Payment} activity, indicating that the appeal has been denied. In contrast, the second example shows that the appeal to the prefecture has been accepted, and no payment is due.

 \begin{table*}[t!]
\caption{Example of generations}\label{tab:generation}
    \centering
    \resizebox{\textwidth}{!}{
        \begin{tabular}{c|l}
            \toprule
            $c$ & trace \\
            \midrule
            F & $\langle$ (Create Fine, 29/12/99) , (Payment, 9/1/00) $\rangle$ \\
            T & $\langle$ (Create Fine, 1/1/00), (Send Fine, 15/4/00), (Insert Fine Notification, 27/4/00), (Appeal to Judge, 27/5/00), (Add penalty, 29/6/00), (Payment, 23/9/01) $\rangle$ \\
            \midrule
            F & $\langle$ (Create Fine, 2/1/00), (Send Fine, 12/3/00), (Payment, 12/4/00) $\rangle$ \\
            T & $\langle$ (Create Fine, 1/1/00), (Send Fine, 15/4/00), (Insert Fine Notification, 29/4/00), (Insert Date Appeal to Prefecture, 6/6/00), (Add penalty, 28/6/00), (Send Appeal to Prefecture, 21/7/00) $\rangle$ \\
            \bottomrule
        \end{tabular}
    }
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We start the analysis of the results by answering \ref{RQ1}. In Figure~\ref{fig:evaluation} we plot the values of the temporal (RED, CTD) and control-flow (2GD) metrics computed for each of the four experiments described in Section~\ref{sec:datasets}.
We can observe that \cvae consistently yields the worst value for the AED metric. This indicates that the overall distributions of all event timestamps in the logs generated by  \lstmi and \lstmii are closer to the one of the test set compared to \cvae.
This can be attributed to two main factors. On one side the \cvae generates traces following the temporal distribution of the training set, which has a temporal horizon four times wider then the one of the test set, thus negatively impacting the AED metric. On the other side, both \lstm models generate all traces very close to initial timestamp provided to start the generation process, bringing them closer to the temporal distribution of the test log. This behaviour is clearly illustrated in Figure~\alert{(da aggiungere!)}.

On the other hand, \cvae consistently outperforms the competing \lstm models in both the cycle time (CTD) and control-flow (2GD) metrics.
It is also worth noting that the \cvae boxplot often overlaps with the \baseline one, indicating that it correctly reproduces the distributions of the training set for this two metrics.
In summary, the quality of the traces generated by the \cvae appears to be much higher than those of the \lstm models. However, further efforts are needed to better reproduce the overall log event temporal distribution measured by the AED metric.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
To address \ref{RQ2}, we report in Table~\ref{tab:variants} the average number of variants generated that already appear in the training or test sets. We observe that, compared to the \lstmi and \lstmii models, which almost always generate new variants, the traces generated by the \cvae model are, depeending on the dataset, \alert{15\% to 77\% already present in the training log and 1\% to 42\% in the test log}. 
Moreover, looking at the CONF values reported in Figure~\ref{fig:evaluation}, we see that \cvae achieves a significantly higher conformance, ranging from 5\% to more than 30\% higher than the \lstm models and very close to the maximal ``self''-conformance value (reached by the \baseline baseline). 
This indicates that almost all the variability generated by the \cvae model complies with the process implicit constraint, while the \lstm models introduce a noticeable degree of non-conformity.
This difference is likely due to the different ``hallucination'' mechanisms used by the two architectures to generate diverse outputs. Specifically, the sampling in the latent space used by the \cvae is more robust compared to the random choice selection of the LSTM network's output used by the \lstm models. The \alert{latter} method has a small but appreciable probability of sampling an incongruous next activity during the trace generation.
\begin{table}[t!]
	\caption{Variant analysis}\label{tab:variants}
	\centering
	\resizebox{.9\columnwidth}{!}{
		\begin{tabular}{l|l|ccc}
			\toprule
			\multirow{2}*{Model} & \multirow{2}*{Dataset}  & Variant \# & Variant \#  &  Variant \#   \\
		&	& (total)  & (in training) & (in test) \\
			\midrule
                \multirow{4}*{\cvae} & \sepsis & 152.7 & 52.8 & 2 \\
                 & \bpia & 880.4 & 125.1 & 43.8 \\
                 & \bpib & 882.2 & 153 & 48.9 \\
                 & \fines & 60.7 & 46.6 & 25.6 \\
                \midrule
                \multirow{4}*{\lstmi} & \sepsis & 157 & 0.1 & 0.1 \\
                  & \bpia  & 937 & 0 & 0 \\
                  & \bpib  & 937 & 0 & 0\\
                  & \fines & 282.7 & 16.1 & 9.8 \\
                \midrule
               \multirow{4}*{\lstmii} & \sepsis & 157 & 0.8 &  0.0\\
                  & \bpia & 936.6 & 1 & 0.6 \\
                  & \bpib & 936.6 & 0.3 & 0.3 \\
                  & \fines & 218.6 & 42 & 26.5 \\
			\bottomrule
		\end{tabular}}
\end{table}


Finally we address \ref{RQ3}.
We report in Table~\ref{tab:conditional_ratio} the conditional ratio of the training, test and the generated logs, computed a-posteriori.
The generated logs should reproduce the ratio appearing in the training set.
We can see that \cvae always reproduce a conditional ratio within 2\% of the training ratio.
This is not the case neither for the \lstmii model, which, even it is trained separately on the two conditioned subset of the log, fails in reproducing the correct ratio for the \sepsis log.
\begin{table}[t!]
\caption{Conditional ratio}\label{tab:conditional_ratio}
    \centering
    %\resizebox{\columnwidth}{!}{
        \begin{tabular}{lccccc}
            \toprule
            dataset & training & test & \cvae & \lstmi & \lstmii  \\
            \midrule
            \sepsis & 14.8\% & 11.5\% & 15\% & 28.6\% & 38.3 \% \\
            \bpia & 16.5\% & 19.2\% & 15.3\% & 14.4\% & 15.1\% \\
            \bpib & 28.2\% & 26\% & 27\% & 31.5\% & 27.3\% \\
            \fines & 3.2\% & 3.6\% & 4\% & 3\% & 4\% \\
            \bottomrule
        \end{tabular}
    %}
\end{table}


